CLEME: Debiasing Multi-reference Evaluation for Grammatical Error Correction

Evaluating the performance of Grammatical Error Correction (GEC) systems is a challenging task due to its subjectivity. Designing an evaluation metric that is as objective as possible is crucial to the development of GEC task. However, mainstream evaluation metrics, i.e., reference-based metrics, introduce bias into the multi-reference evaluation by extracting edits without considering the presence of multiple references. To overcome this issue, we propose Chunk-LEvel Multi-reference Evaluation (CLEME), designed to evaluate GEC systems in the multi-reference evaluation setting. CLEME builds chunk sequences with consistent boundaries for the source, the hypothesis and references, thus eliminating the bias caused by inconsistent edit boundaries. Furthermore, we observe the consistent boundary could also act as the boundary of grammatical errors, based on which the F$_{0.5}$ score is then computed following the correction independence assumption. We conduct experiments on six English reference sets based on the CoNLL-2014 shared task. Extensive experiments and detailed analyses demonstrate the correctness of our discovery and the effectiveness of CLEME. Further analysis reveals that CLEME is robust to evaluate GEC systems across reference sets with varying numbers of references and annotation style.

==> tables/benchmarks.tex <==
\begin{table*}[!tbp]
\centering
\scalebox{1.0}{
\begin{tabular}{llcccc}

\toprule
\multicolumn{1}{c}{\textbf{Language}} & \multicolumn{1}{c}{\textbf{Corpus}} & \textbf{Splits} & \textbf{\# Sents} & \textbf{\# Refs} & \textbf{Domains} \\
\toprule

% English
\multirow{3}{*}{English} & \textbf{CoNLL-2014}~\cite{ng-etal-2014-conll} & Test & 1,312 & 2$\sim$18 & Essays \\

& \textbf{JFLEG}~\cite{napoles-etal-2017-jfleg} & Dev / Test & 754 / 747 & 4 / 4 & Exams \\

& \textbf{BEA-2019}~\cite{bryant-etal-2019-bea} & Train / Dev / Test & 34.3k / 4,384 / 4,477 & 1 / 1 / 5 & Exams, Essays \\

\hline % Chinese
\multirow{3}{*}{Chinese} & \textbf{NLLPCC-2018}~\cite{zhao2018overview} & Train / Test & 717k / 2,000 & 1$\sim$21 / 1$\sim$2 & Web / Essays \\

& \textbf{NLPTEA-2020}~\cite{rao2020overview} & Train / Test & 717k / 1,457 & 1 / 1 & Exams \\

& \textbf{MuCGEC}~\cite{zhang-etal-2022-mucgec} & Dev / Test & 1,125 / 5,938 & 2.3 / 2.3 & Essays, Exams, Web \\

\hline % Czech 
\multirow{2}{*}{Czech} & \textbf{AKCES-GEC}~\cite{naplava-straka-2019-grammatical} & Train / Dev / Test & 42.2k / 2.5k / 2.7k & 1 / 2 / 2 & Essays, Exams \\

& \textbf{GECCC}~\cite{naplava-etal-2022-czech} & Train / Dev / Test & 66.6k / 8.5k / 7.9k & 1 / 1$\sim$2 / 2 & Essays, Exams, Web \\

\hline % Japanese
Japanese & \textbf{TEC-JL}~\cite{koyama-etal-2020-construction} & Test & 1.9k & 2 & Forum \\

\bottomrule
\end{tabular}}
\caption{\label{tab:benchmarks}
Statistics of popular GEC benchmarks.}
\end{table*}

==> tables/details-BN.tex <==
\begin{table*}[htbp!]
\centering
\scalebox{0.88}{
\begin{tabular}{llccccccccccccc}
\toprule

\bf{Metric} &
& \multicolumn{1}{c}{\bf{AMU}}
& \multicolumn{1}{c}{\bf{CAMB}}
& \multicolumn{1}{c}{\bf{CUUI}}
& \multicolumn{1}{c}{\bf{IITB}}
& \multicolumn{1}{c}{\bf{INPUT}}
& \multicolumn{1}{c}{\bf{IPN}}
& \multicolumn{1}{c}{\bf{NTHU}}
& \multicolumn{1}{c}{\bf{PKU}}
& \multicolumn{1}{c}{\bf{POST}}
& \multicolumn{1}{c}{\bf{RAC}}
& \multicolumn{1}{c}{\bf{SJTU}}
& \multicolumn{1}{c}{\bf{UFC}}
& \multicolumn{1}{c}{\bf{UMC}} \\
\hline

\multirow{6}{*}{\bf{ERRANT}} 
& \bf{TP} & 701 & 1100 & 867 & 33 & 0 & 120 & 568 & 426 & 805 & 473 & 150 & 37 & 468 \\
& \bf{FP} & 577 & 954 & 725 & 60 & 0 & 420 & 832 & 565 & 855 & 640 & 215 & 13 & 617 \\
& \bf{FN} & 1560 & 1682 & 1714 & 1481 & 1478 & 1564 & 1622 & 1545 & 1677 & 1590 & 1491 & 1487 & 1599 \\
& \bf{P} & 54.85 & 53.55 & 54.46 & 35.48 & 100.0 & 22.22 & 40.57 & 42.99 & 48.49 & 42.5 & 41.10 & 74.00 & 43.13 \\
& \bf{R} & 31.00 & 39.54 & 33.59 & 2.18 & 0.00 & 7.13 & 25.94 & 21.61 & 32.43 & 22.93 & 9.14 & 2.43 & 22.64 \\
& \bf{F$_{0.5}$} & 47.54 & 50.01 & 48.44 & 8.75 & 0.00 & 15.61 & 36.46 & 35.89 & 44.12 & 36.30 & 24.19 & 10.73 & 36.52 \\

\midrule

\multirow{11}{*}{\bf{CLEME-dependent}}
& \bf{TP} & 436 & 682 & 508 & 21 & 0 & 74 & 333 & 273 & 495 & 287 & 97 & 24 & 324 \\
& \quad w/o LW & 498 & 783 & 604 & 26 & 0 & 74 & 390 & 317 & 579 & 336 & 115 & 31 & 370 \\
& \bf{FP} & 701 & 1093 & 818 & 70 & 0 & 477 & 743 & 645 & 985 & 664 & 247 & 18 & 697 \\
& \quad w/o LW & 668 & 1038 & 785 & 63 & 0 & 449 & 803 & 612 & 937 & 667 & 237 & 19 & 659 \\
& \bf{FN} &844 & 707 & 847 & 1116 & 1135 & 1002 & 822 & 870 & 813 & 864 & 1047 & 1127 & 913 \\
& \quad w/o LW & 930 & 782 & 938 & 1196 & 1217 & 1095 & 912 & 948 & 904 & 946 & 1125 & 1212 & 1005 \\
& \bf{TN} & 10190 & 9822 & 9963 & 10791 & 10832 & 10646 & 10154 & 10346 & 9991 & 10258 & 10648 & 10795 & 10287 \\

& \bf{P} & 38.36 & 38.43 & 38.30 & 23.39 & 100.0 & 13.51 & 28.32 & 29.77 & 33.45 & 30.16 & 28.19 & 56.91 & 31.76 \\
& \bf{R} & 34.08 & 49.11 & 37.48 & 1.88 & 0.00 & 6.92 & 28.84 & 23.92 & 37.84 & 24.92 & 8.47 & 2.09 & 26.21 \\
& \bf{F$_{0.5}$} & 37.42 & 40.18 & 38.14 & 7.11 & 0.00 & 11.35 & 28.42 & 28.38 & 34.24 & 28.94 & 19.23 & 9.12 & 30.47 \\
& \bf{Acc} & 87.31 & 85.38 & 86.28 & 90.12 & 90.51 & 87.88 & 86.30 & 87.52 & 85.36 & 87.34 & 89.25 & 90.42 & 86.83 \\

\hdashline

\multirow{4}{*}{\bf{SentCLEME-dependent}}
& \bf{P} & 70.66 & 53.66 & 65.81 & 95.58 & 100.0 & 68.89 & 59.56 & 68.45 & 62.80 & 69.07 & 84.80 & 98.63 & 68.83 \\
& \bf{R} & 63.00 & 73.92 & 64.98 & 4.87 & 42.76 & 49.48 & 62.79 & 58.43 & 64.85 & 58.83 & 48.11 & 43.64 & 58.22 \\
& \bf{F$_{0.5}$} & 49.83 & 47.36 & 50.27 & 42.59 & 42.76 & 32.54 & 41.87 & 44.24 & 47.65 & 43.66 & 43.39 & 43.48 & 44.66 \\
& \bf{Acc} & 83.59 & 85.09 & 83.97 & 78.01 & 77.74 & 78.17 & 81.97 & 82.01 & 83.30 & 87.97 & 79.40 & 78.11 & 81.76 \\

\midrule

\multirow{11}{*}{\bf{CLEME-independent}}
& \bf{TP} & 452 & 714 & 543 & 21 & 0 & 79 & 343 & 277 & 528 & 302 & 98 & 24 & 338 \\
& \quad w/o LW & 517 & 823 & 648 & 26 & 0 & 78 & 402 & 322 & 619 & 353 & 117 & 31 & 387 \\
& \bf{FP} & 679 & 1045 & 766 & 70 & 0 & 473 & 829 & 638 & 938 & 645 & 244 & 18 & 677 \\
& \quad w/o LW & 649 & 998 & 741 & 63 & 0 & 445 & 791 & 607 & 897 & 650 & 235 & 19 & 642 \\
& \bf{FN} & 466 & 314 & 435 & 790 & 807 & 670 & 472 & 532 & 450 & 524 & 713 & 790 & 547 \\
& \quad w/o LW & 484 & 326 & 453 & 806 & 822 & 696 & 491 & 546 & 475 & 541 & 728 & 805 & 568 \\
& \bf{TN} & 10637 & 10284 & 10454 & 11181 & 11227 & 11045 & 10575 & 10750 & 10431 & 10666 & 11047 & 11202 & 10724 \\

& \bf{P} & 39.98 & 40.60 & 41.51 & 23.39 & 100.0 & 14.32 & 29.27 & 30.26 & 36.02 & 31.86 & 28.71 & 56.91 & 33.32 \\
& \bf{R} & 49.23 & 69.48 & 55.53 & 2.63 & 0.00 & 10.56 & 42.06 & 34.24 & 53.96 & 36.54 & 12.13 & 2.96 & 38.21 \\
& \bf{F$_{0.5}$} & 41.54 & 44.28 & 43.71 & 9.07 & 0.00 & 13.37 & 31.16 & 30.98 & 38.58 & 32.70 & 22.54 & 12.25 & 34.20 \\
& \bf{Acc} & 90.64 & 89.01 & 90.16 & 92.87 & 93.29 & 90.68 & 89.35 & 90.40 & 88.76 & 90.37 & 92.09 & 93.28 & 90.04 \\

\hdashline

\multirow{4}{*}{\bf{SentCLEME-independent}}
& \bf{P} & 72.83 & 57.98 & 69.12 & 95.58 & 100.0 & 68.96 & 61.72 & 69.81 & 6.18 & 70.64 & 85.16 & 98.63 & 70.60 \\
& \bf{R} & 76.92 & 87.02 & 79.84 & 56.57 & 55.26 & 61.97 & 76.56 & 71.94 & 78.83 & 72.28 & 61.39 & 56.80 & 72.05 \\
& \bf{F$_{0.5}$} & 53.03 & 52.74 & 54.38 & 43.76 & 44.13 & 34.21 & 45.73 & 46.43 & 51.92 & 44.59 & 44.75 & 45.17 & 47.08 \\
& \bf{Acc} & 90.91 & 90.26 & 90.75 & 90.67 & 90.89 & 89.16 & 89.52 & 90.26 & 89.91 & 90.14 & 90.59 & 90.97 & 90.01 \\

% & \bf{F$_{0.5}$} & 58.66 & 54.63 & 59.49 & 54.37 & 55.26 & 41.04 & 50.66 & 52.58 & 56.19 & 51.71 & 53.99 & 56.07 & 53.52 \\
% & \bf{Acc} & 92.31 & 91.00 & 92.09 & 92.79 & 93.04 & 90.97 & 90.83 & 91.79 & 91.14 & 91.86 & 92.59 & 93.09 & 91.63 \\

\bottomrule
\end{tabular}}
\caption{\label{tab:details-BN}
A comparison of detailed evaluation results across 13 GEC systems on BN-10GEC~\cite{bryant-ng-2015-far}. We report True Positives (TPs), False Positives (FPs), False Negatives (FNs) and True Negatives (TNs) with or without length weighting (LW).}
\end{table*}

==> tables/details-CoNLL.tex <==
\begin{table*}[tbp!]
\centering
\scalebox{0.9}{
\begin{tabular}{llccccccccccccc}
\toprule
\bf{Metric} &
& \multicolumn{1}{c}{\bf{AMU}}
& \multicolumn{1}{c}{\bf{CAMB}}
& \multicolumn{1}{c}{\bf{CUUI}}
& \multicolumn{1}{c}{\bf{IITB}}
& \multicolumn{1}{c}{\bf{INPUT}}
& \multicolumn{1}{c}{\bf{IPN}}
& \multicolumn{1}{c}{\bf{NTHU}}
& \multicolumn{1}{c}{\bf{PKU}}
& \multicolumn{1}{c}{\bf{POST}}
& \multicolumn{1}{c}{\bf{RAC}}
& \multicolumn{1}{c}{\bf{SJTU}}
& \multicolumn{1}{c}{\bf{UFC}}
& \multicolumn{1}{c}{\bf{UMC}} \\
\hline

\multirow{6}{*}{\bf{ERRANT}} 
& \bf{TP} & 483 & 725 & 607 & 28 & 0 & 52 & 409 & 294 & 508 & 319 & 104 & 36 & 311 \\
& \bf{FP} & 795 & 1329 & 985 & 65 & 0 & 488 & 991 & 697 & 1152 & 794 & 261 & 14 & 774 \\
& \bf{FN} & 1934 & 1886 & 1946 & 2064 & 2070 & 2078 & 1976 & 2007 & 1985 & 2044 & 2036 & 2069 & 2020 \\
& \bf{P} & 37.79 & 35.30 & 38.13 & 30.11 & 100.0 & 9.63 & 29.21 & 29.67 & 30.60 & 28.66 & 28.49 & 72.00 & 28.66 \\
& \bf{R} & 19.98 & 27.77 & 23.78 & 1.34 & 0.00 & 2.44 & 17.15 & 12.78 & 20.38 & 13.50 & 4.86 & 1.71 & 13.34 \\
& \bf{F$_{0.5}$} & 32.08 & 33.48 & 34.02 & 5.68 & 0.00 & 6.06 & 25.61 & 23.46 & 27.81 & 23.40 & 14.44 & 7.81 & 23.31 \\

\midrule

\multirow{11}{*}{\bf{CLEME-dependent}}
& \bf{TP} & 314 & 482 & 379 & 17 & 0 & 33 & 266 & 195 & 333 & 203 & 69 & 24 & 213 \\
& \quad w/o LW & 382 & 588 & 471 & 22 & 0 & 39 & 330 & 246 & 412 & 254 & 85 & 32 & 216 \\
& \bf{FP} & 872 & 1392 & 1034 & 72 & 0 & 529 & 975 & 776 & 1246 & 782 & 292 & 19 & 844 \\
& \quad w/o LW & 815 & 1303 & 964 & 67 & 0 & 488 & 905 & 709 & 1144 & 782 & 272 & 18 & 788 \\
& \bf{FN} & 1182 & 987 & 1169 & 1564 & 1592 & 1445 & 1191 & 1259 & 1158 & 1278 & 1471 & 1583 & 1266 \\
& \quad w/o LW & 1345 & 1132 & 1333 & 1751 & 1782 & 1634 & 1366 & 1426 & 1333 & 1453 & 1657 & 1772 & 1439 \\
& \bf{TN} & 6312 & 6347 & 6245 & 6313 & 6308 & 6412 & 6295 & 6314 & 6449 & 6310 & 6324 & 6280 & 6377 \\

& \bf{P} & 26.45 & 25.74 & 26.81 & 19.29 & 100.0 & 5.85 & 21.42 & 20.06 & 21.07 & 20.60 & 19.02 & 56.40 & 20.14 \\
& \bf{R} & 20.97 & 32.84 & 24.48 & 1.09 & 0.00 & 2.22 & 18.23 & 13.39 & 22.31 & 13.71 & 4.45 & 1.52 & 14.40 \\
& \bf{F$_{0.5}$} & 25.14 & 26.90 & 26.31 & 4.45 & 0.00 & 4.41 & 20.69 & 18.24 & 21.31 & 18.72 & 11.50 & 6.85 & 18.65 \\
& \bf{Acc} & 76.34 & 74.16 & 75.04 & 79.46 & 79.84 & 76.55 & 75.18 & 76.18 & 76.83 & 75.97 & 78.38 & 79.74 & 75.74 \\

\hdashline

\multirow{4}{*}{\bf{SentCLEME-dependent}}
& \bf{P} & 63.05 & 41.07 & 57.60 & 95.27 & 100.0 & 7.45 & 55.17 & 63.62 & 53.26 & 65.05 & 82.90 & 98.70 & 61.78 \\
& \bf{R} & 48.87 & 59.94 & 51.21 & 32.37 & 31.33 & 36.07 & 49.71 & 44.84 & 50.61 & 44.57 & 36.06 & 32.15 & 44.43 \\
& \bf{F$_{0.5}$} & 36.24 & 32.94 & 37.39 & 31.51 & 31.33 & 23.25 & 32.24 & 32.56 & 33.34 & 32.37 & 31.93 & 32.30 & 31.46 \\
& \bf{Acc} & 69.92 & 71.42 & 70.66 & 64.93 & 64.60 & 64.70 & 68.74 & 68.34 & 69.69 & 68.92 & 66.07 & 65.10 & 68.13 \\

\midrule

\multirow{11}{*}{\bf{CLEME-independent}}
& \bf{TP} & 318 & 488 & 392 & 17 & 0 & 33 & 272 & 196 & 339 & 204 & 69 & 24 & 214 \\
& \quad w/o LW & 388 & 596 & 487 & 22 & 0 & 39 & 338 & 248 & 420 & 255 & 85 & 32 & 262 \\
& \bf{FP} & 864 & 1382 & 1016 & 72 & 0 & 529 & 965 & 773 & 1236 & 781 & 292 & 19 & 843 \\
& \quad w/o LW & 809 & 1295 & 948 & 67 & 0 & 488 & 897 & 707 & 1136 & 781 & 272 & 18 & 787 \\                                         
& \bf{FN} & 928 & 701 & 884 & 1362 & 1393 & 1246 & 937 & 1022 & 883 & 1025 & 1266 & 1372 & 1026 \\
& \quad w/o LW & 1029 & 778 & 984 & 1497 & 1530 & 1382 & 1045 & 1129 & 990 & 1135 & 1398 & 1506 & 1136 \\
& \bf{TN} & 6629 & 6701 & 6597 & 6567 & 6560 & 6664 & 6617 & 6611 & 6793 & 6628 & 6583 & 6546 & 6680 \\

& \bf{P} & 26.90 & 26.11 & 27.85 & 19.29 & 100.0 & 5.85 & 22.00 & 20.23 & 21.50 & 20.69 & 19.02 & 56.40 & 20.22 \\
& \bf{R} & 25.53 & 41.06 & 30.71 & 1.25 & 0.00 & 2.57 & 22.52 & 16.10 & 27.72 & 16.59 & 5.14 & 1.75 & 17.23 \\
& \bf{F$_{0.5}$} & 26.61 & 28.16 & 28.38 & 4.97 & 0.00 & 4.66 & 22.10 & 19.24 & 22.51 & 19.71 & 12.35 & 7.77 & 19.54 \\
& \bf{Acc} & 79.50 & 77.53 & 78.63 & 82.11 & 82.48 & 79.05 & 78.37 & 79.13 & 77.10 & 79.09 & 81.02 & 82.52 & 78.67 \\

\hdashline

\multirow{4}{*}{\bf{SentCLEME-independent}}
& \bf{P} & 65.36 & 45.39 & 60.92 & 95.27 & 100.0 & 67.51 & 57.44 & 65.03 & 56.26 & 66.65 & 83.17 & 98.70 & 63.36 \\
& \bf{R} & 57.20 & 70.15 & 60.76 & 36.87 & 35.29 & 40.56 & 58.08 & 52.20 & 59.83 & 52.14 & 41.31 & 36.59 & 51.94 \\
& \bf{F$_{0.5}$} & 42.00 & 39.63 & 43.76 & 35.49 & 35.29 & 25.90 & 38.13 & 37.43 & 39.38 & 37.04 & 36.25 & 36.48 & 36.59 \\
& \bf{Acc} & 76.90 & 77.03 & 77.16 & 75.16 & 75.17 & 73.73 & 75.73 & 75.98 & 76.08 & 76.40 & 75.38 & 75.48 & 75.61 \\

\bottomrule
\end{tabular}}
\caption{\label{tab:details-CoNLL}
A comparison of detailed evaluation results across 13 GEC systems on the CoNLL-2014 shared task. We report True Positives (TPs), False Positives (FPs), False Negatives (FNs) and True Negatives (TNs) with or without length weighting (LW).}
\end{table*}
